Modeling and Controlling Many-Core HPC Processors: an Alternative to PID and Moving Average Algorithms

The race towards performance increase and computing power has led to chips with heterogeneous and complex designs, integrating an ever-growing number of cores on the same monolithic chip or chiplet silicon die. Higher integration density, compounded with the slowdown of technology-driven power reduction, implies that power and thermal management become increasingly relevant. Unfortunately, existing research lacks a detailed analysis and modeling of thermal, power, and electrical coupling effects and how they have to be jointly considered to perform dynamic control of complex and heterogeneous Multi-Processor System on Chips (MPSoCs). To close the gap, in this work, we first provide a detailed thermal and power model targeting a modern High Performance Computing (HPC) MPSoC. We consider real-world coupling effects such as actuators' non-idealities and the exponential relation between the dissipated power, the temperature state, and the voltage level in a single processing element. We analyze how these factors affect the control algorithm behavior and the type of challenges that they pose. Based on the analysis, we propose a thermal capping strategy inspired by Fuzzy control theory to replace the state-of-the-art PID controller, as well as a root-finding iterative method to optimally choose the shared voltage value among cores grouped in the same voltage domain. We evaluate the proposed controller with model-in-the-loop and hardware-in-the-loop co-simulations. We show an improvement over state-of-the-art methods of up to 5x the maximum exceeded temperature while providing an average of 3.56% faster application execution runtime across all the evaluation scenarios.

==> figures/src/ieee_cols.tex <==
\definecolor{ieee-bright-dblue-100}{rgb}{0.0, 0.3828, 0.6055}
\definecolor{ieee-bright-dblue-80}{rgb}{0.0, 0.4883, 0.6797}
\definecolor{ieee-bright-dblue-60}{rgb}{0.3633, 0.6094, 0.7617}
\definecolor{ieee-bright-dblue-40}{rgb}{0.5898, 0.7383, 0.8398}
\definecolor{ieee-bright-dblue-20}{rgb}{0.8906, 0.8984, 0.9219}
\definecolor{ieee-bright-red-100}{rgb}{0.7266, 0.0469, 0.1836}
\definecolor{ieee-bright-red-80}{rgb}{0.832, 0.3164, 0.3281}
\definecolor{ieee-bright-red-60}{rgb}{0.8906, 0.4922, 0.4805}
\definecolor{ieee-bright-red-40}{rgb}{0.9336, 0.6562, 0.6406}
\definecolor{ieee-bright-red-20}{rgb}{0.9688, 0.8203, 0.8125}
\definecolor{ieee-bright-orange-100}{rgb}{0.9961, 0.6367, 0.0}
\definecolor{ieee-bright-orange-80}{rgb}{0.9844, 0.6953, 0.3125}
\definecolor{ieee-bright-orange-60}{rgb}{0.9883, 0.7695, 0.4844}
\definecolor{ieee-bright-orange-40}{rgb}{0.9922, 0.8359, 0.6562}
\definecolor{ieee-bright-orange-20}{rgb}{0.9961, 0.9219, 0.8164}
\definecolor{ieee-bright-yellow-100}{rgb}{0.9961, 0.8164, 0.0}
\definecolor{ieee-bright-yellow-80}{rgb}{0.9961, 0.8477, 0.2148}
\definecolor{ieee-bright-yellow-60}{rgb}{0.9961, 0.875, 0.4492}
\definecolor{ieee-bright-yellow-40}{rgb}{0.9961, 0.9062, 0.6328}
\definecolor{ieee-bright-yellow-20}{rgb}{0.9961, 0.9531, 0.8125}
\definecolor{ieee-bright-lgreen-100}{rgb}{0.4688, 0.7422, 0.125}
\definecolor{ieee-bright-lgreen-80}{rgb}{0.5742, 0.7852, 0.332}
\definecolor{ieee-bright-lgreen-60}{rgb}{0.6875, 0.8398, 0.5039}
\definecolor{ieee-bright-lgreen-40}{rgb}{0.793, 0.8906, 0.6641}
\definecolor{ieee-bright-lgreen-20}{rgb}{0.8945, 0.9414, 0.8281}
\definecolor{ieee-bright-dgreen-100}{rgb}{0.0, 0.5156, 0.2383}
\definecolor{ieee-bright-dgreen-80}{rgb}{0.1641, 0.6055, 0.3867}
\definecolor{ieee-bright-dgreen-60}{rgb}{0.3906, 0.6953, 0.5234}
\definecolor{ieee-bright-dgreen-40}{rgb}{0.6094, 0.8008, 0.6719}
\definecolor{ieee-bright-dgreen-20}{rgb}{0.8047, 0.8945, 0.8359}
\definecolor{ieee-bright-purple-100}{rgb}{0.5938, 0.1133, 0.5898}
\definecolor{ieee-bright-purple-80}{rgb}{0.6992, 0.3281, 0.668}
\definecolor{ieee-bright-purple-60}{rgb}{0.7812, 0.4961, 0.7461}
\definecolor{ieee-bright-purple-40}{rgb}{0.8555, 0.6602, 0.8281}
\definecolor{ieee-bright-purple-20}{rgb}{0.9219, 0.8281, 0.9023}
\definecolor{ieee-bright-lblue-100}{rgb}{0.0, 0.6094, 0.6484}
\definecolor{ieee-bright-lblue-80}{rgb}{0.0, 0.6797, 0.7188}
\definecolor{ieee-bright-lblue-60}{rgb}{0.2109, 0.75, 0.7812}
\definecolor{ieee-bright-lblue-40}{rgb}{0.5469, 0.8242, 0.8438}
\definecolor{ieee-bright-lblue-20}{rgb}{0.7695, 0.918, 0.9219}
\definecolor{ieee-bright-cyan-100}{rgb}{0.0, 0.707, 0.8828}
\definecolor{ieee-bright-cyan-80}{rgb}{0.0, 0.7227, 0.9453}
\definecolor{ieee-bright-cyan-60}{rgb}{0.2656, 0.7812, 0.957}
\definecolor{ieee-bright-cyan-40}{rgb}{0.5547, 0.8438, 0.9688}
\definecolor{ieee-bright-cyan-20}{rgb}{0.7773, 0.9141, 0.9805}
\definecolor{ieee-bright-white-100}{rgb}{0.9961, 0.9961, 0.9961}
\definecolor{ieee-bright-white-80}{rgb}{0.9961, 0.9961, 0.9961}
\definecolor{ieee-bright-white-60}{rgb}{0.9961, 0.9961, 0.9961}
\definecolor{ieee-bright-white-40}{rgb}{0.9961, 0.9961, 0.9961}
\definecolor{ieee-bright-white-20}{rgb}{0.9961, 0.9961, 0.9961}
\definecolor{ieee-dark-red-100}{rgb}{0.5234, 0.1211, 0.2539}
\definecolor{ieee-dark-red-80}{rgb}{0.6445, 0.2812, 0.3828}
\definecolor{ieee-dark-red-60}{rgb}{0.7422, 0.4727, 0.5234}
\definecolor{ieee-dark-red-40}{rgb}{0.832, 0.6445, 0.6758}
\definecolor{ieee-dark-red-20}{rgb}{0.918, 0.8203, 0.832}
\definecolor{ieee-dark-orange-100}{rgb}{0.9062, 0.4648, 0.1328}
\definecolor{ieee-dark-orange-80}{rgb}{0.9648, 0.5664, 0.3164}
\definecolor{ieee-dark-orange-60}{rgb}{0.9766, 0.6758, 0.4805}
\definecolor{ieee-dark-orange-40}{rgb}{0.9844, 0.7773, 0.6523}
\definecolor{ieee-dark-orange-20}{rgb}{0.9922, 0.8789, 0.8125}
\definecolor{ieee-dark-yellow-100}{rgb}{0.9961, 0.7773, 0.1719}
\definecolor{ieee-dark-yellow-80}{rgb}{0.9961, 0.8086, 0.375}
\definecolor{ieee-dark-yellow-60}{rgb}{0.9961, 0.875, 0.4492}
\definecolor{ieee-dark-yellow-40}{rgb}{0.9961, 0.8984, 0.6875}
\definecolor{ieee-dark-yellow-20}{rgb}{0.9961, 0.9453, 0.8438}
\definecolor{ieee-dark-lgreen-100}{rgb}{0.3945, 0.5508, 0.0938}
\definecolor{ieee-dark-lgreen-80}{rgb}{0.5078, 0.6289, 0.293}
\definecolor{ieee-dark-lgreen-60}{rgb}{0.6367, 0.7188, 0.4688}
\definecolor{ieee-dark-lgreen-40}{rgb}{0.7539, 0.8047, 0.6367}
\definecolor{ieee-dark-lgreen-20}{rgb}{0.875, 0.9023, 0.8125}
\definecolor{ieee-dark-dgreen-100}{rgb}{0.0, 0.3867, 0.2539}
\definecolor{ieee-dark-dgreen-80}{rgb}{0.1836, 0.5, 0.3906}
\definecolor{ieee-dark-dgreen-60}{rgb}{0.3984, 0.6172, 0.5273}
\definecolor{ieee-dark-dgreen-40}{rgb}{0.5938, 0.7422, 0.6758}
\definecolor{ieee-dark-dgreen-20}{rgb}{0.793, 0.8711, 0.8359}
\definecolor{ieee-dark-purple-100}{rgb}{0.4648, 0.1445, 0.5117}
\definecolor{ieee-dark-purple-80}{rgb}{0.5898, 0.3242, 0.6016}
\definecolor{ieee-dark-purple-60}{rgb}{0.6914, 0.4883, 0.6953}
\definecolor{ieee-dark-purple-40}{rgb}{0.7969, 0.6523, 0.793}
\definecolor{ieee-dark-purple-20}{rgb}{0.8945, 0.8203, 0.8945}
\definecolor{ieee-dark-cyan-100}{rgb}{0.0, 0.4492, 0.4648}
\definecolor{ieee-dark-cyan-80}{rgb}{0.0, 0.5469, 0.5664}
\definecolor{ieee-dark-cyan-60}{rgb}{0.3047, 0.6602, 0.668}
\definecolor{ieee-dark-cyan-40}{rgb}{0.5586, 0.7695, 0.7734}
\definecolor{ieee-dark-cyan-20}{rgb}{0.7734, 0.8789, 0.8789}
\definecolor{ieee-dark-dblue-100}{rgb}{0.0, 0.1562, 0.332}
\definecolor{ieee-dark-dblue-80}{rgb}{0.1797, 0.3008, 0.4609}
\definecolor{ieee-dark-dblue-60}{rgb}{0.3828, 0.4609, 0.5859}
\definecolor{ieee-dark-dblue-40}{rgb}{0.5781, 0.6289, 0.7188}
\definecolor{ieee-dark-dblue-20}{rgb}{0.7852, 0.8047, 0.8555}
\definecolor{ieee-dark-grey-100}{rgb}{0.457, 0.4688, 0.4805}
\definecolor{ieee-dark-grey-80}{rgb}{0.5625, 0.5625, 0.5742}
\definecolor{ieee-dark-grey-60}{rgb}{0.6641, 0.6641, 0.6758}
\definecolor{ieee-dark-grey-40}{rgb}{0.7734, 0.7695, 0.7773}
\definecolor{ieee-dark-grey-20}{rgb}{0.8789, 0.8828, 0.8828}
\definecolor{ieee-dark-black-100}{rgb}{0.0, 0.0, 0.0}
\definecolor{ieee-dark-black-80}{rgb}{0.3438, 0.3477, 0.3555}
\definecolor{ieee-dark-black-60}{rgb}{0.5, 0.5078, 0.5195}
\definecolor{ieee-dark-black-40}{rgb}{0.6523, 0.6602, 0.6719}
\definecolor{ieee-dark-black-20}{rgb}{0.8164, 0.8242, 0.8281}


==> tables/res_big_tablev1.tex <==
\begin{table}
\centering
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {c=3,r=3}{},
  cell{1}{4} = {c=7}{},
  cell{1}{11} = {c=7}{},
  cell{1}{18} = {c=4}{},
  cell{1}{22} = {c=3}{},
  cell{2}{4} = {c=3}{},
  cell{2}{7} = {c=2}{},
  cell{2}{9} = {r=2}{},
  cell{2}{10} = {r=2}{},
  cell{2}{11} = {c=6}{},
  cell{2}{17} = {r=2}{},
  cell{2}{18} = {r=2}{},
  cell{2}{19} = {r=2}{},
  cell{2}{20} = {r=2}{},
  cell{2}{21} = {r=2}{},
  cell{2}{22} = {r=2}{},
  cell{2}{23} = {r=2}{},
  cell{2}{24} = {r=2}{},
  cell{4}{1} = {r=12}{},
  cell{4}{2} = {r=4}{},
  cell{8}{2} = {r=4}{},
  cell{12}{2} = {r=4}{},
  cell{16}{1} = {r=12}{},
  cell{16}{2} = {r=4}{},
  cell{20}{2} = {r=4}{},
  cell{24}{2} = {r=4}{},
  cell{28}{1} = {r=12}{},
  cell{28}{2} = {r=4}{},
  cell{32}{2} = {r=4}{},
  cell{36}{2} = {r=4}{},
  vlines,
  hline{1,4,16,28,40} = {-}{},
  hline{2} = {4-24}{},
  hline{3} = {4-8,11-16}{},
  hline{5-7,9-11,13-15,17-19,21-23,25-27,29-31,33-35,37-39} = {3-24}{},
  hline{8,12,20,24,32,36} = {2-24}{},
}
Alg1 I Alg2 I Alg3                     &                                     &     & Temperature                          &                                      &                                      &                                          &                                       &                                         &                                         & Power          &          &          &           &             &              &                              & Performance F [GHz] &     &         &     & Performance Execution [\%]~ &         &     \\
                                       &                                     &     & Exceeded Value [°C]                  &                                      &                                      & Time Exceeded                            &                                       & Max [°C]                                & Average [°C]                            & Exceeded Value &          &          &           &             &              & {Total Time \\Exceeded [\%]} & 2-norm              & Max & Average & min & Max                         & Average & min \\
                                       &                                     &     & Max                                  & 95-p                                 & Average                              & Total [s]                                & Average [\%]                          &                                         &                                         & Max [W]        & Max [\%] & 95-p [W] & 95-p [\%] & Average [W] & Average [\%] &                              &                     &     &         &     &                             &         &     \\
\begin{sideways}MAX-WL\end{sideways}   & \begin{sideways}WATER\end{sideways} & 1-D & 0.18 \textbar{} 2.47 \textbar{} 7.73 & 0.18 \textbar{} 1.78 \textbar{} 6.87 & 0.09 \textbar{} 0.45 \textbar{} 3.46 & 0.006 \textbar{} 10.325 \textbar{} 1.643 & 0.01 \textbar{} 14.34 \textbar{} 2.28 & 85.18 \textbar{} 87.47 \textbar{} 92.73 & 63.26 \textbar{} 67.34 \textbar{} 65.23 &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D & 0.42 \textbar{} 2.45 \textbar{} 4.82 & 0.36 \textbar{} 1.53 \textbar{} 4.14 & 0.16 \textbar{} 0.37 \textbar{} 1.91 & 0.025 \textbar{} 11.865 \textbar{} 0.499 & 0.04 \textbar{} 16.48 \textbar{} 0.69 & 85.42 \textbar{} 87.45 \textbar{} 89.82 & 63.68 \textbar{} 67.40 \textbar{} 64.45 &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D & 0.52 \textbar{} 2.41 \textbar{} 4.09 & 0.41 \textbar{} 1.26 \textbar{} 3.64 & 0.17 \textbar{} 0.35 \textbar{} 1.46 & 0.090 \textbar{} 11.998 \textbar{} 0.372 & 0.13 \textbar{} 16.66 \textbar{} 0.52 & 85.52 \textbar{} 87.41 \textbar{} 89.09 & 63.23 \textbar{} 67.44 \textbar{} 64.22 &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D & 0.65 \textbar{} 2.44 \textbar{} 1.04 & 0.46 \textbar{} 0.94 \textbar{} 0.83 & 0.17 \textbar{} 0.35 \textbar{} 0.38 & 0.298 \textbar{} 11.027 \textbar{} 0.211 & 0.41 \textbar{} 15.32 \textbar{} 0.29 & 85.65 \textbar{} 87.44 \textbar{} 86.04 & 63.47 \textbar{} 67.82 \textbar{} 64.35 &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       & \begin{sideways}AIR\end{sideways}   & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       & \begin{sideways}RACK\end{sideways}  & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
\begin{sideways}MULTI-WL\end{sideways} & \begin{sideways}WATER\end{sideways} & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       & \begin{sideways}AIR\end{sideways}   & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       & \begin{sideways}RACK\end{sideways}  & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
\begin{sideways}CLOUD-WL\end{sideways} & \begin{sideways}WATER\end{sideways} & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       & \begin{sideways}AIR\end{sideways}   & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       & \begin{sideways}RACK\end{sideways}  & 1-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 4-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & 9-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     \\
                                       &                                     & A-D &                                      &                                      &                                      &                                          &                                       &                                         &                                         &                &          &          &           &             &              &                              &                     &     &         &     &                             &         &     
\end{tblr}
\end{table}


==> tables/res_fin.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\definecolor{Green}{rgb}{0,0.901,0}
\definecolor{Red}{rgb}{0.949,0,0}
\begin{table}
\centering
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {r=3}{},
  cell{1}{2} = {c=5}{},
  cell{1}{7} = {c=5}{},
  cell{1}{12} = {c=4}{},
  cell{2}{2} = {c=2}{},
  cell{2}{4} = {c=2}{},
  cell{2}{7} = {c=2}{},
  cell{2}{9} = {c=2}{},
  cell{2}{11} = {r=2}{},
  cell{2}{12} = {c=2}{},
  cell{2}{14} = {c=2}{},
  cell{4}{2} = {Green},
  cell{4}{3} = {Green},
  cell{4}{4} = {Green},
  cell{4}{5} = {Green},
  cell{4}{6} = {Green},
  cell{4}{7} = {Green},
  cell{4}{8} = {Green},
  cell{4}{9} = {Green},
  cell{4}{10} = {Green},
  cell{4}{11} = {Green},
  cell{4}{12} = {yellow},
  cell{4}{13} = {yellow},
  cell{4}{14} = {Red},
  cell{4}{15} = {Red},
  cell{5}{2} = {Red},
  cell{5}{3} = {Red},
  cell{5}{4} = {Red},
  cell{5}{5} = {yellow},
  cell{5}{6} = {Red},
  cell{5}{7} = {yellow},
  cell{5}{8} = {yellow},
  cell{5}{9} = {Red},
  cell{5}{10} = {Red},
  cell{5}{11} = {Red},
  cell{5}{12} = {Red},
  cell{5}{13} = {Red},
  cell{5}{14} = {Green},
  cell{5}{15} = {Green},
  cell{6}{2} = {yellow},
  cell{6}{3} = {yellow},
  cell{6}{4} = {yellow},
  cell{6}{5} = {Red},
  cell{6}{6} = {yellow},
  cell{6}{7} = {Red},
  cell{6}{8} = {Red},
  cell{6}{9} = {yellow},
  cell{6}{10} = {yellow},
  cell{6}{11} = {yellow},
  cell{6}{12} = {Green},
  cell{6}{13} = {Green},
  cell{6}{14} = {yellow},
  cell{6}{15} = {yellow},
  vlines,
  hline{1,4-7} = {-}{},
  hline{2} = {2-15}{},
  hline{3} = {2-10,12-15}{},
}
Alg          & \textbf{Performance}    &             &                        &              &                     & \textbf{Temperature}                                   &             &                             &             &                                                & \textbf{Power}                  &             &                             &             \\
             & \textbf{2-norm [GHz/t]} &             & \textbf{AV-Wl\_p [\%]} &              & \textbf{Wl\_p~[\%]} & \textbf{Exceeded Max Value [\textbackslash{}degree C]} &             & \textbf{Exceeded Time [\%]} &             & \textbf{ Average T [\textbackslash{}degree C]} & \textbf{Exceeded Av Value [\%]} &             & \textbf{Exceeded Time [\%]} &             \\
             & \textbf{Av~}            & \textbf{SD} & \textbf{Av}            & \textbf{SD~} & \textbf{2-norm~}    & \textbf{Max~}                                          & \textbf{Av} & \textbf{Av}                 & \textbf{SD} &                                                & \textbf{Av~}                    & \textbf{SD} & \textbf{Av}                 & \textbf{SD} \\
\textbf{FCA} & 32.05                   & 48.64       & 81.64                  & 7.24         & 0.71                & 2.31                                                   & 0.71        & 0.42                        & 0.64        & 58.21                                          & 3.19                            & 2.99        & 2.33                        & 5.92        \\
\textbf{OCA} & 39.56                   & 61.10       & 79.27                  & 9.24         & 1.66                & 3.63                                                   & 2.25        & 28.14                       & 13.91       & 62.64                                          & 11.07                           & 8.65        & 1.30                        & 0.44        \\
\textbf{VBA} & 39.34                   & 59.86       & 79.84                  & 9.92         & 1.35                & 18.01                                                  & 4.25        & 3.80                        & 4.55        & 60.15                                          & 1.30                            & 1.08        & 1.83                        & 1.69        
\end{tblr}
\end{table}
